Hypergraph Partitioning through Vertex Separators on Graphs

The modeling flexibility provided by hypergraphs has drawn a lot of interest from the combinatorial scientific community, leading to novel models and algorithms, their applications, and development of associated tools. Hypergraphs are now a standard tool in combinatorial scientific computing. The modeling flexibility of hypergraphs however, comes at a cost: algorithms on hypergraphs are inherently more complicated than those on graphs, which sometimes translate to nontrivial increases in processing times. Neither the modeling flexibility of hypergraphs, nor the runtime efficiency of graph algorithms can be overlooked. Therefore, the new research thrust should be how to cleverly trade-off between the two. This work addresses one method for this trade-off by solving the hypergraph partitioning problem by finding vertex separators on graphs. Specifically, we investigate how to solve the hypergraph partitioning problem by seeking a vertex separator on its net intersection graph (NIG), where each net of the hypergraph is represented by a vertex, and two vertices share an edge if their nets have a common vertex. We propose a vertex-weighting scheme to attain good node-balanced hypergraphs, since NIG model cannot preserve node balancing information. Vertex-removal and vertex-splitting techniques are described to optimize cutnet and connectivity metrics, respectively, under the recursive bipartitioning paradigm. We also developed an implementation for our GPVS-based HP formulations by adopting and modifying a state-of-the-art GPVS tool onmetis. Experiments conducted on a large collection of sparse matrices confirmed the validity of our proposed techniques.

==> conclusions.tex <==
\section {Conclusions}

%We have  presented how  the hypergraph partitioning problem can be  efficiently and effectively solved  through finding vertex separators on  the net  intersection graph  representation of a hypergraph. 
%Our  empirical study on a wide set of test matrices showed that  runtimes can be  as much as 4.17 times faster, with the cutsize quality is preserved on average (and improved in many cases), while  balance was achieved for small number of parts and remained acceptable for large number of parts. Moreover, we proposed techniques  that can trade off  cutsize and runtime against balance, showing that balance can be achieved even for high number of parts. 
%Overall results prove that, the proposed hypergraph partitioning  through vertex separators on graphs  is ideal for applications where balance is not well-defined, which is the main motivation for our work, and competitive for application where  balance is important. 

%We believe that the success of the proposed methods  point to several  future research directions.  First,  better vertex weighting schemes to approximate the node balance  is an area that can make a significant impact. We believe  exploiting domain specific information or devising techniques  that can apply  to certain classes of graphs, as opposed to constructing generic approximations that can work  for all graphs, is a promising avenue to explore.  Secondly,  the algorithms we have used in this paper,  were only slightly adjusted for  the particular problem we were solving.  There is a lot of room for improvements in algorithms for finding vertex separators  with balanced hypergraph partitions, and we believe these algorithms can be designed and implemented  on the  existing partitioning  graph partitioning frameworks, which means strong algorithmic ideas can be translated into effective software tools with relatively little effort.   Finally, this paper is only an example of the growing importance of graph partitioning and the need for  more flexible models for graph partitioning. Graph partitioning now is an internal step for divide-and-conquer based methods, whose popularity will only increase with the growing problems sizes.  As such, requirements for  graph partitioning will keep growing and broadening.   While, the state of the art  for graph partitioning  has drastically improved from the days of merely minimizing the number of cut edges, while keeping the number of vertices balanced between the {\it two} parts, we believe  there is  still a lot of room for growth for more general models for graph partitioning. 

\label{sec-conc}
We have presented how the hypergraph partitioning problem can be
efficiently and effectively solved through finding vertex separators
on the net intersection graph representation of a hypergraph.  Our
empirical study on a wide set of test matrices showed that runtimes
can be as much as 4.17 times faster, with the cutsize quality is
preserved on average (and improved in many cases), while balance was
achieved for small number of parts and remained acceptable for large
number of parts. Moreover, we proposed techniques that can trade off
cutsize and runtime against balance, showing that balance can be
achieved even for high number of parts.  Overall results prove that,
the proposed hypergraph partitioning through vertex separators on
graphs is ideal for applications where balance is not well-defined,
which is the main motivation for our work, and competitive for
application where balance is important.

We believe that the success of the proposed methods point to several
future research directions.  First, better vertex weighting schemes to
approximate the node balance is an area that can make a significant
impact. We believe exploiting domain specific information or devising
techniques that can apply to certain classes of graphs, as opposed to
constructing generic approximations that can work for all graphs, is a
promising avenue to explore.  Secondly, the algorithms we have used in
this paper, were only slightly adjusted for the particular problem we
were solving.  There is a lot of room for improvements in algorithms
for finding vertex separators with balanced hypergraph partitions, and
we believe these algorithms can be designed and implemented on the
existing partitioning graph partitioning frameworks, which means
strong algorithmic ideas can be translated into effective software
tools with relatively little effort.  Finally, this paper is only an
example of the growing importance of graph partitioning and the need
for more flexible models for graph partitioning. Graph partitioning
now is an internal step for divide-and-conquer based methods, whose
popularity will only increase with the growing problems sizes.  As
such, requirements for graph partitioning will keep growing and
broadening.  While, the state of the art for graph partitioning has
drastically improved from the days of merely minimizing the number of
cut edges, while keeping the number of vertices balanced between the
{\it two} parts, we believe there is still a lot of room for growth
for more general models for graph partitioning.



==> introduction.tex <==
%
\section{Introduction}
%
A hypergraph is a generalization of a graph, since it replaces edges
that connect only two vertices, with hyperedges (nets) that can connect
multiple vertices.  This generalization  provides a critical modeling
flexibility that allows accurate formulation of many  important
problems in combinatorial scientific computing.  
Our initial motivations for hypergraph models were accurate modeling of the nonzero
structure of unsymmetric and rectangular sparse matrices to minimize communication volume 
for iterative solvers~\cite{Catalyurek96,Catalyurek99,Catalyurek01B,
Catalyurek01C,Catalyurek10-SISC, Dingle04, Bisseling06, Ucar04, Ucar07sisc,
Ucar06sirev, Malas06, vastenhouw05} and permutation to 
block-angular form for coarse-grain parallelism~\cite{Aykanat04}. 
The real impact of these works turned out to be the introduction of
hypergraph models to the combinatorial scientific computing community.  
Since then, the modeling power of hypergraphs appealed to many researchers and was applied to a wide variety of
parallel and distributed computing applications such as data aggregation~\cite{CHANG01B}, 
image-space parallel direct volume rendering~\cite{Cambazoglu07},
parallel mixed integer linear programming~\cite{Szederkenyi10},
data declustering for multi-disk databases~\cite{Koyuturk05, Liu01},
scheduling file-sharing tasks in heterogeneous master-slave computing environments~\cite{Kaya06,Kaya07,Khanna05},
and work-stealing scheduling~\cite{Vrba09}.
Hypergraphs were also applied to applications outside the parallel computing domain such as road network clustering 
for efficient query processing~\cite{Demir10a,Demir08,Demir10b}, 
pattern-based data clustering~\cite{Ozdal04}, reducing software development and maintenance costs~\cite{Bisseling05},
processing spatial join operations~\cite{Shekhar02}, and
improving locality in memory or cache performance~\cite{Akbudak10, strout04, Yzelman09}.
Hypergraphs and hypergraph partitioning are now standard tools of combinatorial scientific computing.

Increasing popularity of hypergraphs  has been going hand in hand with the
development of effective hypergraph partitioning (HP) tools: 
wide applicability of hypergraphs motivated development of fast HP tools, 
and availability of effective HP tools motivated further applications. 
 This virtuous cycle produced sequential HP tools such as
 hMeTiS~\cite{hmetismanual}, PaToH~\cite{patohmanual} and
 Mondriaan~\cite{vastenhouw05},  and parallel HP tools such as
 Parkway~\cite{Trifunovic04c} and Zoltan~\cite{Devine06},
 all of which adopt the multilevel  framework successfully.  
While these tools provide good performances both in terms of solution quality and processing times,
 they are hindered by the inherent complexity of  dealing with hypergraphs.
 Algorithms on hypergraphs are more difficult both in terms of computational
complexity and runtime performance, since operations on nets are
performed on sets of vertices as opposed to pairs of vertices as in
graphs. The wide interest  over the last decade has proven the modeling 
flexibility of hypergraphs to be essential, but the runtime efficiency
of graph algorithms cannot be overlooked, either.  
 Therefore, we believe that  the new research thrust should be how to cleverly
 trade-off between  the modeling flexibility of  hypergraphs and the practicality of graphs. 

How can we solve problems that are most accurately modeled with hypergraphs 
using graph algorithms without sacrificing too much from what is really important for the application? 
This question has been asked before, and the motivation was 
either theoretical~\cite{Ihler93} or  practical~\cite{ChScZi93,HaMaVa92}
when  the absence of HP tools  behest these attempts.  
This earlier body of work investigated the relation between
  HP and graph partitioning by edge separator (GPES), and achieved little success.  
 Today, we are facing a more difficult task, as effectiveness of available 
 HP tools sets high standards for novel approaches.  
On the other hand, we can draw upon the progress on 
 related problems, in particular the advances 
 in tools for graph partitioning by vertex separator (GPVS), which is the main theme of this work. 

We investigate solving the HP problem by finding
vertex separator on the {\it net intersection graph} ({\sc NIG}) of
the hypergraph. In the {\sc NIG}of a hypergraph, each net is represented by a vertex and and each vertex of
the hypergraph is replaced with a clique of the nets connecting that vertex.  
%An example of a NIG of a hypergraph is illustrated in Figure~\ref{}.  
A vertex separator on this graph defines a net separator for the
hypergraph.  This model has been initially studied for circuit
partitioning~\cite{Alpert95}.  While faster algorithms can be designed to find vertex
separators on graphs, the {\sc NIG} model has the drawback of
attaining balanced partitions.  Once vertices of the hypergraphs are
replaced with cliques, it will be impossible to preserve the vertex
weight information accurately.  Therefore, we can view the {\sc NIG}
model as a way to trade off computational efficiency with exact
modeling power.

What motivates us to investigate NIGs to solve
HP problems arising in scientific computing
applications is that in many applications, definition of balance cannot
be very precise~\cite{Aykanat04, Pinar97, Pinar96} or there are additional constraints that cannot be 
easily incorporated into partitioning algorithms and
tools~\cite{pinar01irregular}; or partitioning is
used as part of  a divide-and-conquer
algorithm~\cite{pinar06ETNA}. For 
instance, hypergraph models can be used to permute a linear program
(LP) constraint matrix to a block angular form for parallel solution
with decomposition methods.  Load balance can be achieved by balancing
subproblems during partitioning. However, it is not possible to
accurately predict solution time of an LP, and equal sized subproblems
only increase the likelihood of computational balance. Hypergraph models
have recently been used to find null-space bases that have a sparse
inverse~\cite{pinar06ETNA}. This application requires finding a column-space basis $B$ as
a submatrix of a sparse matrix $A$, so that $B^{-1}$ is
sparse. Choosing $B$ to have a block angular form limits the fill in
$B^{-1}$, but merely a block angular form for $B$ will not be
sufficient, since $B$ has to be nonsingular
to be a column-space basis for $A$.  Enforcing numerical or even structural nonsingularity of
subblocks during partitioning is a nontrivial task, if possible, and
thus partitioning is used as part of a divide-and-conquer paradigm,
where the partitioning phase is followed by a correction phase, if
subblocks are non-singular. Both of these cases present examples of
applications, where hypergraphs provide effective models, but balance
among parts is only weakly defined. As we will show in the
experiments, the {\sc NIG} model can effectively be employed for these
applications to achieve high quality solutions in a shorter time.
We show that it is easy to enforce a balance criteria on the internal nets of hypergraph
partitioning by enforcing vertex balancing during the partitioning of the NIG.
However, the NIG model cannot completely preserve the
node balancing information in the hypergraph. 
We propose a weighting scheme for the vertices of NIG, which is quite effective
in attaining fairly node balanced partitions of the hypergraph.
The proposed vertex balancing scheme for NIG partitioning can be easily enhanced to 
improve the balancing quality of the hypergraph partitions in a simple post processing phase. 


%%ALI PINAR
%We also show that although the NIG model cannot completely preserve the balance
%information in the hypergraph, our approximation techniques are queite effective in 
%attaining fairly balanced paratiions that can be easily enhanced to balanced partitions 
%in a simple post processing phase.

The recursive bipartitioning (RB) paradigm is widely used for multiway
HP and known to produce good solution qualities~\cite{patohmanual, hmetismanual}.
At each RB step, cutnet removal and cutnet splitting techniques~\cite{Catalyurek99}
are adopted to optimize the cutsize according to the {\em cutnet} and {\em connectivity} metrics,
respectively, which are the most commonly used cutsize metrics in 
scientific and parallel computing~\cite{Aykanat04,Catalyurek99} as
well as VLSI layout design~\cite{Alpert95, Lengauer90}.
In this paper, we propose separator-vertex removal and separator-vertex splitting 
techniques for RB-based partitioning of the NIG, 
which exactly correspond to the cutnet removal and cutnet splitting techniques, respectively.
We also propose an implementation for our GPVS-based HP formulations by adopting and modifying a 
state-of-the-art GPVS tool used in fill-reducing sparse matrix ordering.

%The remainder of this paper is organized as follows.  Section~\ref{sec-prelim} presents the preliminaries for this paper,
% which include definitions for the GPES, GPVS and HP problems.  Section~\ref{sec-nig} discusses the proposed GPVS-based HP formulations and  implementation.
% Section~\ref{sec-tools} contains a brief
% review of the recent and successful graph and
% HP algorithms and tools.
%Section~\ref{sec-results} presents our experimental results, and we conclude with Section~\ref{sec-conc}.




